Feeding of active galactic nuclei by dynamical perturbations

There possibly was an AGN episode in the Galactic Centre about 6 Myr ago, powerful enough to produce the Fermi bubbles. We present numerical simulations of a possible scenario giving rise to an activity episode: a collision between a central gas ring surrounding the supermassive black hole (SMBH) and an infalling molecular cloud. We investigate different initial collision angles between the cloud and the ring. We follow the hydrodynamical evolution of the system following the collision using Gadget-3 hybrid N-body/SPH code and calculate the feeding rate of the SMBH accretion disc. This rate is then used as an input for a 1D thin $\alpha$-disc model in order to calculate the AGN luminosity. By varying the disc feeding radii we determine the limiting values for possible AGN accretion disc luminosity. Small angle collisions do not result in significant mass transport to the centre of the system, while models with highest collision angles transport close to $40\%$ of the initial matter to the accretion disc. Even with ring and cloud masses equal to $10^4 \, M_\odot$, which is the lower limit of present-day mass of the Circumnuclear ring in the Galactic Centre, the energy released over an interval of 1.5 Myr can produce $\sim 10\%$ of that required to inflate the Fermi bubbles. If the gas ring in the Galactic Centre 6 Myr ago had a mass of at least $10^5 \, M_\odot$, our proposed scenario can explain the formation of the Fermi bubbles. We estimate that such high-impact collisions might occur once every $\sim 10^8$ yr in our Galaxy.

==> AGN feeding by cloud smashing (1)/Atsakymas.tex <==

> I believe that this study represents an interesting attempt to explain (and possibly connect) several features observed in the Centre of our Galaxy. Even though some of their claims might be a bit speculative, I appreciate that the authors always tried to justify these with qualitatively and often quantitatively arguments. Few concerns from my side will follow, but I would suggest the publication of the present manuscript, after minor/moderate revision.

We thank the reviewer for the comments. The reviewer raised some important points and suggested additional simulations that make our conclusions more robust. We have addressed all the comments. The edits are marked in green in the updated manuscript.

We address each point in order:

> 1. In particular, my main concern is related to the assumption for the size/mass of the cloud. The authors adopted a size of 1 pc and a mass of 10^4 Msun, citing Kauffmann et al. (2017). However, typically larger and more massive clouds are observed by these authors. This is also the case of the +20 and +50 km/s clouds, that are by some authors in the literature believed to be at distances comparable to those adopted in this study. The size of the cloud, in particular, might be affecting (perhaps crucially) the results of this study. The paper would benefit of few additional simulations exploring these parameters (especially the cloud radius), as in the case of Section 4.2 and Fig. 12 for the cloud/ring mass ratio.

We chose the lower estimate of CNR mass and assume the mass of the cloud to be the same. This allows us to determine the lower limit of accretion at a given collision angle. As our model is scale free, we can extrapolate up to higher masses. And, given that our results are not very sensitive to the ring/cloud mass ratio, they can be applied to more realistic larger cloud masses as well.

The point about the radius of the cloud is important as, following Kauffmann et al. (2017), the cloud radius increases along with mass. We carried out several simulations with varied cloud radius, similarly to those with varied cloud mass. Their results are presented in fig. 13 and section 4.2. In general, the effect of changing the cloud radius by a factor two produces negligible differences to total accretion rates.

Larger clouds, both in mass and diameter as well as the +20 and +50 km/s clouds will be the focus of future work. 

> 2. Another possible concern might be related to inclusion of the gravitational potential of the nuclear star clusters. In fact, as shown in Fritz et al. (2016), its enclosed mass becomes comparable to the mass of the central SMBH, at distances of the order of 3-4 pc. Hence, this might have an effect on the tidal deformation of the cloud, before the ring-cloud collision, possibly having an impact of the results. However, I do not suggest the authors to rerun all the simulations of the present study, but rather to consider this for possible follow-up studies.

In addition to the SMBH’s, an isothermal potential, that encloses somewhat more mass in given radius, is used in our models. We mentioned this previously in Section 2.1 but now describe the properties of the potential in more detail. In particular, the enclosed mass is equal to the mass of the SMBH at a distance of 0.8 pc. This is less than the 3-4 pc estimated by Fritz et al. (2016) because our potential includes dark matter and gas as well as stars.


> Few small additional comments/suggestions:
> 3. - In the Introduction, along with the result about the gamma-ray (Fermi) bubbles, the authors might cite the very recent results about the X-ray chimney by Ponti et al. (2019) and the radio bubbles by Heywood et al. (2019).

Citations for the new observations are now included in section 1.

> 4. - In the Introduction, the works by Bonnell & Rice (2008) and Hobbs & Nayakshin (2009), related to the subject of star formation from a disrupted molecular cloud, are mentioned. It would be fair to also briefly acknowledge similar studies, e.g., by Alig et al. (2011, 2013) and Lucas (2013).

Suggested citations are now included in section 1. Alig et al. (2013) is also cited in section 4.6 as the result of creating both misaligned rings and considerable accretion with single CNR/cloud collision is similar to our own.

> 5. - M in Equation 8 and Fig. 9 should be Macc.

Both instances have been corrected.

> 6. - At the end of section 3.4 there is a long segment of text that is repeated. This should be removed.

Removed the repeated segment of text.

> 7. - In section 4.6 the authors acknowledge the work of Bartko et al. (2009), suggesting the presence of two counter-rotating disks of young stars in the central 0.5 pc. However, the more recent work by Yelda et al. (2014) disputes this result.  The authors should acknowledge this.

Yelda et al. (2014) is now cited and the disputed existence of one of the rings is highlighted.

> 8. - In section 4.7 there is a strange sentence starting with "I think it's better to say that...". Please check and correct this.

Segment of the paragraph is now corrected.

> 9. - There are few additional typos, please go through the text again.

We tried to correct as many mistakes as we found.

> 10. - Please make sure that all the plots are easily readable also by colour blind people. This does not seem to be the case for most of the plots. E.g., try to use different linestyles for different curves in the same plot.

Plots were remade with different linestyles where appropriate.

==> Atsakymas.tex <==

> I believe that this study represents an interesting attempt to explain (and possibly connect) several features observed in the Centre of our Galaxy. Even though some of their claims might be a bit speculative, I appreciate that the authors always tried to justify these with qualitatively and often quantitatively arguments. Few concerns from my side will follow, but I would suggest the publication of the present manuscript, after minor/moderate revision.

We thank the reviewer for the comments. The reviewer raised some important points and suggested additional simulations that make our conclusions more robust. We have addressed all the comments. The edits are marked in green in the updated manuscript.

We address each point in order:

> 1. In particular, my main concern is related to the assumption for the size/mass of the cloud. The authors adopted a size of 1 pc and a mass of 10^4 Msun, citing Kauffmann et al. (2017). However, typically larger and more massive clouds are observed by these authors. This is also the case of the +20 and +50 km/s clouds, that are by some authors in the literature believed to be at distances comparable to those adopted in this study. The size of the cloud, in particular, might be affecting (perhaps crucially) the results of this study. The paper would benefit of few additional simulations exploring these parameters (especially the cloud radius), as in the case of Section 4.2 and Fig. 12 for the cloud/ring mass ratio.

We chose the lower estimate of CNR mass and assume the mass of the cloud to be the same. This allows us to determine the lower limit of accretion at a given collision angle. As our model is scale free, we can extrapolate up to higher masses. And, given that our results are not very sensitive to the ring/cloud mass ratio, they can be applied to more realistic larger cloud masses as well.

The point about the radius of the cloud is important as, following Kauffmann et al. (2017), the cloud radius increases along with mass. We carried out several simulations with varied cloud radius, similarly to those with varied cloud mass. Their results are presented in fig. 13 and section 4.2. In general, the effect of changing the cloud radius by a factor two produces negligible differences to total accretion rates.

Larger clouds, both in mass and diameter as well as the +20 and +50 km/s clouds will be the focus of future work. 

> 2. Another possible concern might be related to inclusion of the gravitational potential of the nuclear star clusters. In fact, as shown in Fritz et al. (2016), its enclosed mass becomes comparable to the mass of the central SMBH, at distances of the order of 3-4 pc. Hence, this might have an effect on the tidal deformation of the cloud, before the ring-cloud collision, possibly having an impact of the results. However, I do not suggest the authors to rerun all the simulations of the present study, but rather to consider this for possible follow-up studies.

In addition to the SMBH’s, an isothermal potential, that encloses somewhat more mass in given radius, is used in our models. We mentioned this previously in Section 2.1 but now describe the properties of the potential in more detail. In particular, the enclosed mass is equal to the mass of the SMBH at a distance of 0.8 pc. This is less than the 3-4 pc estimated by Fritz et al. (2016) because our potential includes dark matter and gas as well as stars.


> Few small additional comments/suggestions:
> 3. - In the Introduction, along with the result about the gamma-ray (Fermi) bubbles, the authors might cite the very recent results about the X-ray chimney by Ponti et al. (2019) and the radio bubbles by Heywood et al. (2019).

Citations for the new observations are now included in section 1.

> 4. - In the Introduction, the works by Bonnell & Rice (2008) and Hobbs & Nayakshin (2009), related to the subject of star formation from a disrupted molecular cloud, are mentioned. It would be fair to also briefly acknowledge similar studies, e.g., by Alig et al. (2011, 2013) and Lucas (2013).

Suggested citations are now included in section 1. Alig et al. (2013) is also cited in section 4.6 as the result of creating both misaligned rings and considerable accretion with single CNR/cloud collision is similar to our own.

> 5. - M in Equation 8 and Fig. 9 should be Macc.

Both instances have been corrected.

> 6. - At the end of section 3.4 there is a long segment of text that is repeated. This should be removed.

Removed the repeated segment of text.

> 7. - In section 4.6 the authors acknowledge the work of Bartko et al. (2009), suggesting the presence of two counter-rotating disks of young stars in the central 0.5 pc. However, the more recent work by Yelda et al. (2014) disputes this result.  The authors should acknowledge this.

Yelda et al. (2014) is now cited and the disputed existence of one of the rings is highlighted.

> 8. - In section 4.7 there is a strange sentence starting with "I think it's better to say that...". Please check and correct this.

Segment of the paragraph is now corrected.

> 9. - There are few additional typos, please go through the text again.

We tried to correct as many mistakes as we found.

> 10. - Please make sure that all the plots are easily readable also by colour blind people. This does not seem to be the case for most of the plots. E.g., try to use different linestyles for different curves in the same plot.

Plots were remade with different linestyles where appropriate.
